Fast and Accurate Dual-Way Streaming PARAFAC2 for Irregular Tensors -- Algorithm and Application

How can we efficiently and accurately analyze an irregular tensor in a dual-way streaming setting where the sizes of two dimensions of the tensor increase over time? What types of anomalies are there in the dual-way streaming setting? An irregular tensor is a collection of matrices whose column lengths are the same while their row lengths are different. In a dual-way streaming setting, both new rows of existing matrices and new matrices arrive over time. PARAFAC2 decomposition is a crucial tool for analyzing irregular tensors. Although real-time analysis is necessary in the dual-way streaming, static PARAFAC2 decomposition methods fail to efficiently work in this setting since they perform PARAFAC2 decomposition for accumulated tensors whenever new data arrive. Existing streaming PARAFAC2 decomposition methods work in a limited setting and fail to handle new rows of matrices efficiently. In this paper, we propose Dash, an efficient and accurate PARAFAC2 decomposition method working in the dual-way streaming setting. When new data are given, Dash efficiently performs PARAFAC2 decomposition by carefully dividing the terms related to old and new data and avoiding naive computations involved with old data. Furthermore, applying a forgetting factor makes Dash follow recent movements. Extensive experiments show that Dash achieves up to 14.0x faster speed than existing PARAFAC2 decomposition methods for newly arrived data. We also provide discoveries for detecting anomalies in real-world datasets, including Subprime Mortgage Crisis and COVID-19.

==> 070application.tex <==


\begin{table*}[t!]
%	\vspace{-2mm}
	\caption{Description of real-world tensor datasets.
%	in $\mathbb{R}^{t \times c}$ where $t$ corresponds to total length (time), and $c$ corresponds to the number of time series.
	}
	\centering
	\label{tab:Description}
		\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lrrrrrrrc}
		\toprule
		& \multicolumn{3}{c}{\textbf{Total Tensor Size}} & \multicolumn{3}{c}{\textbf{Initial Tensor Size}} & \\
		\textbf{Dataset} & \textbf{Max Dim. $I_k$} & \textbf{Dim. $J$} & \textbf{Dim. $K$} & \textbf{Max Dim. $I_k$} & \textbf{Dim. $J$} & \textbf{Dim. $K$} & \textbf{Update Cycle} & \textbf{Newly Arrived Data} \\
		\midrule
%		 Brainq\footnoteref{foot:brainq}~\cite{MitchellT2008Predicting}  & $3$ & $(360, 21764, 9)$ & $(10, 10, 5)$ \\
		US Stock~\cite{JangK22} &  $7,397$ & $85$ & $4,742$ &  $1,458$ & $85$ & $994$ & 60 days & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}New rows of existing slice matrices \\ and new slice matrices \blue{arrive}\end{tabular}} \\
		KR Stock~\cite{JangK21} &  $5,268$ & $85$ & $3,620$ &  $995$ & $85$ & $2,092$ & 60 days  \\
		\midrule
		JPN Stock &  $2,204$ & $85$ & $215$ &  $424$ & $85$ & $215$  & 20 days & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}New rows of \\ existing slice matrices \blue{arrive}\end{tabular}} \\
		CHN Stock &  $2,431$ & $85$ & $219$ &  $471$ & $85$ & $219$  & 20 days \\						
		VicRoads~\cite{schimbinschi2015traffic} &  $1,084$ & $96$ & $2,033$ &  $184$ & $96$ & $2,033$  & 20 days \\					
		PEMS &  $440$ & $144$ & $963$ &  $80$ & $144$ & $963$  & 20 days \\						
		\bottomrule
	\end{tabular}}
\end{table*}



What anomalies exist in a dual-way streaming setting?
How can we find them using \method?
As new rows of slice matrices and new slice matrices \blue{arrive} over time, various anomalies are hidden in the new ones.
Although factor matrices are updated using the new incoming data, anomalies are still very different from predictions by the updated factor matrices.
\method efficiently finds anomalies by measuring reconstruction errors with updated factor matrices.

\blue{We find two types of anomaly detection in our dual-way streaming setting:}
\begin{enumerate}
%	\item \textbf{Element-level anomaly detection.} We measure element-wise reconstruction errors and then find an update cycle that provokes \blue{a large error} from the previous update.
	\item \textbf{Slice-level anomaly detection.}	 For a slice matrix, we measure slice matrix-wise reconstruction errors and then find \blue{an update that provokes a large error.}
	\item \textbf{Tensor-level anomaly detection.}	 We measure the reconstruction error for a newly arrived tensor and then compare it \blue{with a threshold.}
\end{enumerate}


%
%\textbf{Element-level anomaly detection.}
%We find element-level anomalies by measuring reconstruction errors of elements of a new incoming tensor and comparing them.
%\blue{For an element, we regard the updates that have high reconstruction errors as anomalies.}
%The following definition is an element-level reconstruction error used for detecting element-level anomalies:
%\begin{definition}[Element-level reconstruction error]
%		When a new element $\mat{X}_{k,new}(i,j)$ is given, an element-level reconstruction error is as follows:
%\blue{\begin{align}
%	ee\left(\mat{X}_{k,new}(i,j)\right) = |\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|
%\end{align}
%where $|\mat{X}(i,j)-\hat{\mat{X}}(i,j)|$ indicates the absolute value of $\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)$.}
%\end{definition}

\textbf{Slice-level anomaly detection.}
\blue{
We find slice-level anomalies by measuring reconstruction errors of slice matrices and investigating them independently.}
We compute reconstruction errors of slice matrices based on the following definition:
\begin{definition}[Slice-level reconstruction error]
\label{def:slice_level}
		When a newly arrived slice matrix $\mat{X}_{k,new}$ is given, a slice-level reconstruction error is as follows:
\blue{
\begin{align}
	se\left(\mat{X}_{k,new}\right) = \frac{1}{I_{k,new}\times J}{\sum_{i,j}{{|\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|}}}
\end{align}
where $\hat{\mat{X}}_{k,new}$ is the reconstructed matrix by $\mat{U}_{k,new}\mat{S}_{k,new}\mat{V}_{new}^T$.
}
\end{definition}




\textbf{Tensor-level anomaly detection.}
We detect tensor-level anomalies by measuring a reconstruction error for a newly arrived tensor.
There are newly arrived tensors that fail to be reconstructed well.
\blue{When a new tensor arrives}, we obtain a reconstruction error by updating factor matrices and comparing the new one with the reconstructed data by the updated factor matrices.
Then, we compare it with reconstruction errors measured at previous updates.
The following definition presents the tensor-level reconstruction error:
\begin{definition}[Tensor-level reconstruction error]
\label{def:tensor_level}
		When a newly arrived tensor $\T{X}_{new} = \{\mat{X}_{k,new}\}_{k=1}^{K+L}$ is given, tensor-level reconstruction error is as follows:
\blue{
\begin{align}
\begin{split}
	& te\left(\{\mat{X}_{k,new}\}_{k=1}^{K+L}\right) = \\
	&  \frac{1}{K+L}\sum_{k=1}^{K+L}\frac{1}{I_{k,new}\times J}{\sum_{i,j}{|\mat{X}_{k,new}(i,j)-\hat{\mat{X}}_{k,new}(i,j)|}}
\end{split}
\end{align}
where $\hat{\mat{X}}_{k,new}$ is reconstructed by $\mat{U}_{k,new}\mat{S}_{k,new}\mat{V}_{new}^T$.
}
\end{definition}

After measuring reconstruction errors, we identify the updates with \blue{high reconstruction errors} above a threshold as abnormal.
%When a newly arrived tensor is different from factor matrices of an accumulated tensor, high reconstruction errors occur.





